Low-frequency radio spectra of submillimetre galaxies in the Lockman Hole

We investigate the radio properties of a sample of 53 sources selected at 850 $\mu$m from the SCUBA-2 Cosmology Legacy Survey using new deep, low-frequency radio imaging of the Lockman Hole field from the Low Frequency Array. Combining these data with additional radio observations from the GMRT and the JVLA, we find a variety of radio spectral shapes and luminosities within our sample despite their similarly bright submillimetre flux densities. We characterise their spectral shapes in terms of multi-band radio spectral indices. Finding strong spectral flattening at low frequencies in ~20% of sources, we investigate the differences between sources with extremely flat low-frequency spectra and those with `normal' radio spectral indices. As there are no other statistically significant differences between the two subgroups of our sample as split by the radio spectral index, we suggest that any differences are undetectable in galaxy-averaged properties that we can observe with our unresolved images, and likely relate to galaxy properties that we cannot resolve, on scales $\lesssim$ 1 kpc. We attribute the observed spectral flattening in the radio to free-free absorption, proposing that those sources with significant low-frequency spectral flattening have a clumpy distribution of star-forming gas. We estimate an average spatial extent of absorbing material of at most several hundred parsecs to produce the levels of absorption observed in the radio spectra. This estimate is consistent with the highest-resolution observations of submillimetre galaxies in the literature, which find examples of non-uniform dust distributions on scales of ~100 pc, with evidence for clumps and knots in the interstellar medium. Additionally, we find two bright (> 6 mJy) submm sources undetected at all other wavelengths. We speculate that these objects may be very high redshift sources, likely residing at z > 4.

==> table1.tex <==
ID	&	RA 	&	Dec	&	S$_{850} $	&	S$_{150 \rm{MHz}} $	&	S$_{324 \rm{MHz}} $	&	S$_{610 \rm{MHz}} $	&	S$_{1.4 \rm{GHz}} $	&	$\alpha_{150-324}$	&	$\alpha_{324-1400}$	& z	&		\\  
		& 		&		&		(mJy)	&	($\mu$Jy)		&	($\mu$Jy)		&	($\mu$Jy)		&	($\mu$Jy)		&						&						&	&		\\  
\hline 
1  	&	$10^{\mathrm{h}}46^{\mathrm{m}}35.78^{\mathrm{s}}$	&	$+59^{\circ} 7{'}48.00{''}$	&	11.91	&	$560.73$	&	$269.05$	&	$215.36$	&	$80.64$	&	$-0.91$	&	$-0.82$	&	$1.89$\\ 
2  	&	$10^{\mathrm{h}}46^{\mathrm{m}}45.01^{\mathrm{s}}$	&	$+59^{\circ}15{'}39.80{''}$	&	12.28	&	$619.46$	&	$326.56$	&	$230.62$	&	$60.12$	&	$-0.80$	&	$-1.16$	&	$1.30$\\ 
3* 	&	$10^{\mathrm{h}}47^{\mathrm{m}}27.66^{\mathrm{s}}$	&	$+58^{\circ}52{'}14.60{''}$	&	9.91	&	$475.02$	&	$218.79$	&	$243.83$	&	$76.62$	&	$-0.96$	&	$-0.72$	&	$2.93$\\ 
4  	&	$10^{\mathrm{h}}47^{\mathrm{m}}0.03^{\mathrm{s}}$	&	$+59^{\circ} 1{'}7.50{''}$	&	8.92	&	$682.39$	&	$654.40$	&	$463.67$	&	$232.95$	&	$-0.05$	&	$-0.71$	&	$2.73$\\ 
5  	&	$10^{\mathrm{h}}45^{\mathrm{m}}35.23^{\mathrm{s}}$	&	$+58^{\circ}50{'}49.90{''}$	&	8.66	&	$283.04$	&	$185.44$	&	$97.98$	&	$46.60$	&	$-0.53$	&	$-0.94$	&	$3.76$\\ 
6  	&	$10^{\mathrm{h}}45^{\mathrm{m}}55.19^{\mathrm{s}}$	&	$+59^{\circ}15{'}28.10{''}$	&	9.68	&	$168.58$	&	$226.77$	&	$66.25$	&	$32.53$	&	$0.37$	&	$-1.33$	&	$4.48$\\ 
7  	&	$10^{\mathrm{h}}46^{\mathrm{m}}32.85^{\mathrm{s}}$	&	$+59^{\circ} 2{'}12.00{''}$	&	8.15	&	$464.85$	&	$318.65$	&	$217.56$	&	$119.51$	&	$-0.47$	&	$-0.67$	&	$3.42$\\ 
8 $^{\dagger}$	&	$10^{\mathrm{h}}45^{\mathrm{m}}54.58^{\mathrm{s}}$	&	$+58^{\circ}47{'}54.10{''}$	&	8.31	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
9* 	&	$10^{\mathrm{h}}47^{\mathrm{m}}25.25^{\mathrm{s}}$	&	$+59^{\circ} 3{'}40.70{''}$	&	7.92	&	$382.96$	&	$242.35$	&	$110.80$	&	$36.95$	&	$-0.57$	&	$-1.29$	&	$2.32$\\ 
10  	&	$10^{\mathrm{h}}46^{\mathrm{m}}31.68^{\mathrm{s}}$	&	$+58^{\circ}50{'}54.00{''}$	&	7.91	&	$2997.08$	&	$1591.78$	&	$923.99$	&	$265.02$	&	$-0.79$	&	$-1.23$	&	$  -  $\\ 
11  	&	$10^{\mathrm{h}}48^{\mathrm{m}}3.37^{\mathrm{s}}$	&	$+58^{\circ}54{'}22.90{''}$	&	8.92	&	$3154.12$	&	$1886.64$	&	$965.98$	&	$261.03$	&	$-0.64$	&	$-1.35$	&	$2.66$\\ 
12  	&	$10^{\mathrm{h}}44^{\mathrm{m}}47.69^{\mathrm{s}}$	&	$+59^{\circ} 0{'}36.60{''}$	&	7.45	&	$968.78$	&	$597.49$	&	$314.52$	&	$131.48$	&	$-0.60$	&	$-1.03$	&	$1.98$\\ 
13  	&	$10^{\mathrm{h}}47^{\mathrm{m}}20.57^{\mathrm{s}}$	&	$+59^{\circ}10{'}40.90{''}$	&	7.35	&	$736.93$	&	$399.62$	&	$218.91$	&	$65.99$	&	$-0.76$	&	$-1.23$	&	$2.69$\\ 
14  	&	$10^{\mathrm{h}}46^{\mathrm{m}}57.26^{\mathrm{s}}$	&	$+59^{\circ}14{'}57.60{''}$	&	7.87	&	$416.05$	&	$211.55$	&	$173.30$	&	$34.05$	&	$-0.84$	&	$-1.25$	&	$2.96$\\ 
15  	&	$10^{\mathrm{h}}44^{\mathrm{m}}56.86^{\mathrm{s}}$	&	$+58^{\circ}49{'}59.00{''}$	&	7.56	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
16 $^{\dagger}$	&	$10^{\mathrm{h}}45^{\mathrm{m}}1.83^{\mathrm{s}}$	&	$+59^{\circ} 4{'}3.10{''}$	&	6.81	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
17* 	&	$10^{\mathrm{h}}47^{\mathrm{m}}18.21^{\mathrm{s}}$	&	$+59^{\circ} 2{'}31.00{''}$	&	6.77	&	$430.70$	&	$230.10$	&	$155.23$	&	$39.92$	&	$-0.78$	&	$-1.20$	&	$2.31$\\ 
18  	&	$10^{\mathrm{h}}45^{\mathrm{m}}56.87^{\mathrm{s}}$	&	$+58^{\circ}53{'}18.10{''}$	&	6.76	&	$854.53$	&	$611.55$	&	$413.93$	&	$205.57$	&	$-0.42$	&	$-0.74$	&	$1.39$\\ 
19  	&	$10^{\mathrm{h}}47^{\mathrm{m}}2.61^{\mathrm{s}}$	&	$+58^{\circ}51{'}5.40{''}$	&	6.72	&	$279.62$	&	$304.00$	&	$68.13$	&	$31.74$	&	$0.10$	&	$-1.54$	&	$3.28$\\ 
20  	&	$10^{\mathrm{h}}48^{\mathrm{m}}1.05^{\mathrm{s}}$	&	$+59^{\circ} 3{'}43.10{''}$	&	7.45	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
21  	&	$10^{\mathrm{h}}46^{\mathrm{m}}33.24^{\mathrm{s}}$	&	$+58^{\circ}52{'}0.00{''}$	&	6.45	&	$268.16$	&	$170.03$	&	$129.69$	&	$55.18$	&	$-0.57$	&	$-0.77$	&	$3.00$\\ 
22* 	&	$10^{\mathrm{h}}45^{\mathrm{m}}23.87^{\mathrm{s}}$	&	$+59^{\circ}16{'}25.70{''}$	&	8.25	&	$651.38$	&	$349.86$	&	$187.96$	&	$30.08$	&	$-0.77$	&	$-1.68$	&	$0.82$\\ 
23  	&	$10^{\mathrm{h}}43^{\mathrm{m}}51.48^{\mathrm{s}}$	&	$+59^{\circ} 0{'}57.70{''}$	&	8.15	&	$333.42$	&	$302.24$	&	$123.97$	&	$36.63$	&	$-0.12$	&	$-1.44$	&	$2.27$\\ 
24* 	&	$10^{\mathrm{h}}46^{\mathrm{m}}26.92^{\mathrm{s}}$	&	$+59^{\circ} 5{'}44.10{''}$	&	6.47	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
25  	&	$10^{\mathrm{h}}44^{\mathrm{m}}40.23^{\mathrm{s}}$	&	$+58^{\circ}59{'}28.30{''}$	&	6.31	&	$559.67$	&	$248.83$	&	$191.35$	&	$67.50$	&	$-1.01$	&	$-0.89$	&	$2.14$\\ 
26* 	&	$10^{\mathrm{h}}47^{\mathrm{m}}15.49^{\mathrm{s}}$	&	$+59^{\circ} 6{'}33.10{''}$	&	6.50	&	$343.77$	&	$200.46$	&	$148.73$	&	$45.82$	&	$-0.67$	&	$-1.01$	&	$3.95$\\ 
27*$^{\dagger}$	&	$10^{\mathrm{h}}47^{\mathrm{m}}20.94^{\mathrm{s}}$	&	$+58^{\circ}51{'}52.90{''}$	&	6.32	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
28  	&	$10^{\mathrm{h}}46^{\mathrm{m}}32.97^{\mathrm{s}}$	&	$+59^{\circ}12{'}20.00{''}$	&	6.17	&	$304.81$	&	$134.93$	&	$122.89$	&	$47.90$	&	$-1.01$	&	$-0.71$	&	$2.61$\\ 
29  	&	$10^{\mathrm{h}}45^{\mathrm{m}}22.55^{\mathrm{s}}$	&	$+59^{\circ}17{'}21.70{''}$	&	8.84	&	$454.25$	&	$208.33$	&	$196.16$	&	$55.21$	&	$-0.97$	&	$-0.91$	&	$1.99$\\ 
30 $^{\dagger}$	&	$10^{\mathrm{h}}48^{\mathrm{m}}0.04^{\mathrm{s}}$	&	$+58^{\circ}54{'}47.10{''}$	&	6.42	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
31  	&	$10^{\mathrm{h}}48^{\mathrm{m}}13.49^{\mathrm{s}}$	&	$+59^{\circ} 3{'}38.30{''}$	&	6.69	&	$233.08$	&	$203.56$	&	$77.61$	&	$25.53$	&	$-0.17$	&	$-1.42$	&	$3.19$\\ 
32* 	&	$10^{\mathrm{h}}46^{\mathrm{m}}31.00^{\mathrm{s}}$	&	$+58^{\circ}59{'}8.00{''}$	&	5.52	&	$215.21$	&	$186.59$	&	$105.71$	&	$32.39$	&	$-0.18$	&	$-1.20$	&	$5.64$\\ 
33  	&	$10^{\mathrm{h}}47^{\mathrm{m}}34.22^{\mathrm{s}}$	&	$+59^{\circ}13{'}28.40{''}$	&	6.30	&	$347.99$	&	$182.35$	&	$111.52$	&	$45.49$	&	$-0.80$	&	$-0.95$	&	$3.15$\\ 
34* 	&	$10^{\mathrm{h}}47^{\mathrm{m}}18.23^{\mathrm{s}}$	&	$+58^{\circ}55{'}25.00{''}$	&	5.44	&	$243.85$	&	$245.03$	&	$56.77$	&	$39.70$	&	$0.01$	&	$-1.24$	&	$3.84$\\ 
35  	&	$10^{\mathrm{h}}46^{\mathrm{m}}38.72^{\mathrm{s}}$	&	$+58^{\circ}56{'}11.90{''}$	&	5.50	&	$656.21$	&	$367.44$	&	$283.81$	&	$129.00$	&	$-0.72$	&	$-0.72$	&	$2.27$\\ 
36  	&	$10^{\mathrm{h}}46^{\mathrm{m}}59.87^{\mathrm{s}}$	&	$+58^{\circ}54{'}37.50{''}$	&	5.42	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
37 $^{\dagger}$	&	$10^{\mathrm{h}}46^{\mathrm{m}}23.24^{\mathrm{s}}$	&	$+58^{\circ}59{'}36.10{''}$	&	4.86	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
38  	&	$10^{\mathrm{h}}48^{\mathrm{m}}22.92^{\mathrm{s}}$	&	$+59^{\circ} 1{'}9.70{''}$	&	6.37	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
39  	&	$10^{\mathrm{h}}44^{\mathrm{m}}31.37^{\mathrm{s}}$	&	$+59^{\circ} 6{'}15.90{''}$	&	4.98	&	$315.48$	&	$315.02$	&	$153.90$	&	$53.63$	&	$-0.00$	&	$-1.21$	&	$1.14$\\ 
40 $^{\dagger}$	&	$10^{\mathrm{h}}44^{\mathrm{m}}42.19^{\mathrm{s}}$	&	$+59^{\circ} 2{'}10.40{''}$	&	5.07	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
41  	&	$10^{\mathrm{h}}46^{\mathrm{m}}8.49^{\mathrm{s}}$	&	$+58^{\circ}58{'}28.20{''}$	&	5.05	&	$1387.43$	&	$786.63$	&	$447.18$	&	$189.72$	&	$-0.71$	&	$-0.97$	&	$2.09$\\ 
42  	&	$10^{\mathrm{h}}44^{\mathrm{m}}30.59^{\mathrm{s}}$	&	$+58^{\circ}55{'}15.90{''}$	&	5.25	&	$517.03$	&	$181.98$	&	$192.92$	&	$44.27$	&	$-1.30$	&	$-0.97$	&	$1.94$\\ 
43  	&	$10^{\mathrm{h}}47^{\mathrm{m}}30.73^{\mathrm{s}}$	&	$+59^{\circ} 4{'}22.50{''}$	&	5.02	&	$371.09$	&	$331.18$	&	$162.85$	&	$65.27$	&	$-0.14$	&	$-1.11$	&	$1.76$\\ 
44  	&	$10^{\mathrm{h}}46^{\mathrm{m}}1.99^{\mathrm{s}}$	&	$+59^{\circ} 9{'}18.20{''}$	&	4.73	&	$505.02$	&	$345.32$	&	$193.13$	&	$64.20$	&	$-0.47$	&	$-1.15$	&	$1.88$\\ 
45  	&	$10^{\mathrm{h}}47^{\mathrm{m}}29.72^{\mathrm{s}}$	&	$+59^{\circ}11{'}32.50{''}$	&	5.31	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
46  	&	$10^{\mathrm{h}}46^{\mathrm{m}}1.26^{\mathrm{s}}$	&	$+58^{\circ}51{'}52.20{''}$	&	4.53	&	$561.38$	&	$297.33$	&	$222.81$	&	$116.54$	&	$-0.79$	&	$-0.64$	&	$2.27$\\ 
47 $^{\dagger}$	&	$10^{\mathrm{h}}46^{\mathrm{m}}21.39^{\mathrm{s}}$	&	$+58^{\circ}54{'}34.10{''}$	&	4.66	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
48 $^{\dagger}$	&	$10^{\mathrm{h}}44^{\mathrm{m}}18.32^{\mathrm{s}}$	&	$+59^{\circ} 2{'}41.30{''}$	&	5.00	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
49  	&	$10^{\mathrm{h}}47^{\mathrm{m}}44.16^{\mathrm{s}}$	&	$+59^{\circ}14{'}11.90{''}$	&	5.89	&	$214.73$	&	$150.22$	&	$104.23$	&	$40.82$	&	$-0.44$	&	$-0.89$	&	$2.20$\\ 
50  	&	$10^{\mathrm{h}}44^{\mathrm{m}}44.53^{\mathrm{s}}$	&	$+59^{\circ}14{'}50.50{''}$	&	6.40	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
51* 	&	$10^{\mathrm{h}}43^{\mathrm{m}}55.28^{\mathrm{s}}$	&	$+59^{\circ} 6{'}16.00{''}$	&	6.04	&	$360.91$	&	$231.01$	&	$145.52$	&	$51.86$	&	$-0.55$	&	$-1.02$	&	$2.84$\\ 
52  	&	$10^{\mathrm{h}}45^{\mathrm{m}}39.90^{\mathrm{s}}$	&	$+58^{\circ}48{'}30.00{''}$	&	4.60	&	$351.83$	&	$252.34$	&	$187.14$	&	$67.46$	&	$-0.41$	&	$-0.90$	&	$3.70$\\ 
53  	&	$10^{\mathrm{h}}47^{\mathrm{m}}37.65^{\mathrm{s}}$	&	$+58^{\circ}56{'}32.20{''}$	&	4.59	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $	&	$  -  $\\ 
\hline 


==> table_IDs.tex <==
ID	& LOFAR source ID 	&	RA 	&	Dec	&	z	\\  
\hline 
1  	&	ILTJ104635.83+590749.2	&	$10^{\mathrm{h}}46^{\mathrm{m}}35.78^{\mathrm{s}}$	&	$+59^{\circ} 7{'}48.00{''}$	&	$1.89$$\pm^{0.71}_{0.68}$\\ 
2  	&	ILTJ104644.98+591542.4	&	$10^{\mathrm{h}}46^{\mathrm{m}}45.01^{\mathrm{s}}$	&	$+59^{\circ}15{'}39.80{''}$	&	$1.30$$\pm^{0.92}_{1.08}$\\ 
3* 	&	ILTJ104727.95+585213.9	&	$10^{\mathrm{h}}47^{\mathrm{m}}27.66^{\mathrm{s}}$	&	$+58^{\circ}52{'}14.60{''}$	&	$2.93$$\pm^{0.39}_{0.42}$\\ 
4  	&	ILTJ104700.22+590108.1	&	$10^{\mathrm{h}}47^{\mathrm{m}}0.03^{\mathrm{s}}$	&	$+59^{\circ} 1{'}7.50{''}$	&	$2.73$$\pm^{0.48}_{0.57}$\\ 
5  	&	ILTJ104535.03+585050.1	&	$10^{\mathrm{h}}45^{\mathrm{m}}35.23^{\mathrm{s}}$	&	$+58^{\circ}50{'}49.90{''}$	&	$3.76$$\pm^{0.89}_{0.86}$\\ 
6  	&	ILTJ104555.38+591528.7	&	$10^{\mathrm{h}}45^{\mathrm{m}}55.19^{\mathrm{s}}$	&	$+59^{\circ}15{'}28.10{''}$	&	$4.48$$\pm^{2.72}_{2.52}$\\ 
7  	&	ILTJ104632.77+590214.3	&	$10^{\mathrm{h}}46^{\mathrm{m}}32.85^{\mathrm{s}}$	&	$+59^{\circ} 2{'}12.00{''}$	&	$3.42$$\pm^{1.34}_{1.38}$\\ 
8 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}45^{\mathrm{m}}54.58^{\mathrm{s}}$	&	$+58^{\circ}47{'}54.10{''}$	&	$  -  $ \\ 
9* 	&	ILTJ104725.39+590337.8	&	$10^{\mathrm{h}}47^{\mathrm{m}}25.25^{\mathrm{s}}$	&	$+59^{\circ} 3{'}40.70{''}$	&	$2.32$$\pm^{0.74}_{0.80}$\\ 
10  	&	ILTJ104631.52+585055.9	&	$10^{\mathrm{h}}46^{\mathrm{m}}31.68^{\mathrm{s}}$	&	$+58^{\circ}50{'}54.00{''}$	&	$  -  $\\ 
11  	&	ILTJ104803.58+585421.4	&	$10^{\mathrm{h}}48^{\mathrm{m}}3.37^{\mathrm{s}}$	&	$+58^{\circ}54{'}22.90{''}$	&	$2.66$$\pm^{0.49}_{0.50}$\\ 
12  	&	ILTJ104447.60+590035.5	&	$10^{\mathrm{h}}44^{\mathrm{m}}47.69^{\mathrm{s}}$	&	$+59^{\circ} 0{'}36.60{''}$	&	$1.98$$\pm^{0.69}_{0.78}$\\ 
13  	&	ILTJ104720.51+591043.6	&	$10^{\mathrm{h}}47^{\mathrm{m}}20.57^{\mathrm{s}}$	&	$+59^{\circ}10{'}40.90{''}$	&	$2.69$$\pm^{0.80}_{0.66}$\\ 
14  	&	ILTJ104657.32+591459.2	&	$10^{\mathrm{h}}46^{\mathrm{m}}57.26^{\mathrm{s}}$	&	$+59^{\circ}14{'}57.60{''}$	&	$2.96$$\pm^{0.75}_{0.62}$\\ 
15  	&	ILTJ104456.67+585000.0	&	$10^{\mathrm{h}}44^{\mathrm{m}}56.86^{\mathrm{s}}$	&	$+58^{\circ}49{'}59.00{''}$	&	$  -  $ \\ 
16 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}45^{\mathrm{m}}1.83^{\mathrm{s}}$	&	$+59^{\circ} 4{'}3.10{''}$	&	$  -  $ \\ 
17* 	&	ILTJ104717.95+590232.2	&	$10^{\mathrm{h}}47^{\mathrm{m}}18.21^{\mathrm{s}}$	&	$+59^{\circ} 2{'}31.00{''}$	&	$2.31$$\pm^{0.34}_{0.39}$\\ 
18  	&	ILTJ104556.88+585318.8	&	$10^{\mathrm{h}}45^{\mathrm{m}}56.87^{\mathrm{s}}$	&	$+58^{\circ}53{'}18.10{''}$	&	$1.39$$\pm^{0.64}_{0.68}$\\ 
19  	&	ILTJ104702.46+585102.9	&	$10^{\mathrm{h}}47^{\mathrm{m}}2.61^{\mathrm{s}}$	&	$+58^{\circ}51{'}5.40{''}$	&	$3.28$$\pm^{1.89}_{1.86}$\\ 
20  	&	ILTJ104800.86+590343.8	&	$10^{\mathrm{h}}48^{\mathrm{m}}1.05^{\mathrm{s}}$	&	$+59^{\circ} 3{'}43.10{''}$	&	$  -  $ \\ 
21  	&	ILTJ104633.12+585158.7	&	$10^{\mathrm{h}}46^{\mathrm{m}}33.24^{\mathrm{s}}$	&	$+58^{\circ}52{'}0.00{''}$	&	$3.00$$\pm^{1.16}_{1.14}$\\ 
22* 	&	ILTJ104523.51+591631.2	&	$10^{\mathrm{h}}45^{\mathrm{m}}23.87^{\mathrm{s}}$	&	$+59^{\circ}16{'}25.70{''}$	&	$0.82$$\pm^{0.20}_{0.16}$\\ 
23  	&	ILTJ104351.14+590058.1	&	$10^{\mathrm{h}}43^{\mathrm{m}}51.48^{\mathrm{s}}$	&	$+59^{\circ} 0{'}57.70{''}$	&	$2.27$$\pm^{0.56}_{0.60}$\\ 
24* 	&	ILTJ104626.25+590539.5	&	$10^{\mathrm{h}}46^{\mathrm{m}}26.92^{\mathrm{s}}$	&	$+59^{\circ} 5{'}44.10{''}$	&	$  -  $ \\ 
25  	&	ILTJ104440.17+585929.8	&	$10^{\mathrm{h}}44^{\mathrm{m}}40.23^{\mathrm{s}}$	&	$+58^{\circ}59{'}28.30{''}$	&	$2.14$$\pm^{0.74}_{1.37}$\\ 
26* 	&	ILTJ104715.52+590636.6	&	$10^{\mathrm{h}}47^{\mathrm{m}}15.49^{\mathrm{s}}$	&	$+59^{\circ} 6{'}33.10{''}$	&	$3.95$$\pm^{2.06}_{2.14}$\\ 
27*$^{\dagger}$	&	 	&	$10^{\mathrm{h}}47^{\mathrm{m}}20.94^{\mathrm{s}}$	&	$+58^{\circ}51{'}52.90{''}$	&	$  -  $ \\ 
28  	&	ILTJ104633.11+591220.2	&	$10^{\mathrm{h}}46^{\mathrm{m}}32.97^{\mathrm{s}}$	&	$+59^{\circ}12{'}20.00{''}$	&	$2.61$$\pm^{1.19}_{1.09}$\\ 
29  	&	ILTJ104522.33+591726.0	&	$10^{\mathrm{h}}45^{\mathrm{m}}22.55^{\mathrm{s}}$	&	$+59^{\circ}17{'}21.70{''}$	&	$1.99$$\pm^{0.76}_{0.74}$\\ 
30 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}48^{\mathrm{m}}0.04^{\mathrm{s}}$	&	$+58^{\circ}54{'}47.10{''}$	&	$  -  $ \\ 
31  	&	ILTJ104813.45+590340.9	&	$10^{\mathrm{h}}48^{\mathrm{m}}13.49^{\mathrm{s}}$	&	$+59^{\circ} 3{'}38.30{''}$	&	$3.19$$\pm^{2.12}_{2.14}$\\ 
32* 	&	ILTJ104630.75+585908.3	&	$10^{\mathrm{h}}46^{\mathrm{m}}31.00^{\mathrm{s}}$	&	$+58^{\circ}59{'}8.00{''}$	&	$5.64$$\pm^{1.17}_{1.08}$\\ 
33  	&	ILTJ104734.49+591333.2	&	$10^{\mathrm{h}}47^{\mathrm{m}}34.22^{\mathrm{s}}$	&	$+59^{\circ}13{'}28.40{''}$	&	$3.15$$\pm^{1.97}_{2.06}$\\ 
34* 	&	ILTJ104718.16+585525.9	&	$10^{\mathrm{h}}47^{\mathrm{m}}18.23^{\mathrm{s}}$	&	$+58^{\circ}55{'}25.00{''}$	&	$3.84$$\pm^{1.23}_{1.34}$\\ 
35  	&	ILTJ104638.62+585612.6	&	$10^{\mathrm{h}}46^{\mathrm{m}}38.72^{\mathrm{s}}$	&	$+58^{\circ}56{'}11.90{''}$	&	$2.27$$\pm^{0.32}_{0.33}$\\ 
36  	&	ILTJ104700.07+585441.5	&	$10^{\mathrm{h}}46^{\mathrm{m}}59.87^{\mathrm{s}}$	&	$+58^{\circ}54{'}37.50{''}$	&	$  -  $ \\ 
37 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}46^{\mathrm{m}}23.24^{\mathrm{s}}$	&	$+58^{\circ}59{'}36.10{''}$	&	$  -  $ \\ 
38  	&	ILTJ104822.99+590112.1	&	$10^{\mathrm{h}}48^{\mathrm{m}}22.92^{\mathrm{s}}$	&	$+59^{\circ} 1{'}9.70{''}$	&	$  -  $ \\ 
39  	&	ILTJ104431.34+590612.8	&	$10^{\mathrm{h}}44^{\mathrm{m}}31.37^{\mathrm{s}}$	&	$+59^{\circ} 6{'}15.90{''}$	&	$1.14$$\pm^{0.16}_{0.15}$\\ 
40 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}44^{\mathrm{m}}42.19^{\mathrm{s}}$	&	$+59^{\circ} 2{'}10.40{''}$	&	$  -  $ \\ 
41  	&	ILTJ104608.72+585828.7	&	$10^{\mathrm{h}}46^{\mathrm{m}}8.49^{\mathrm{s}}$	&	$+58^{\circ}58{'}28.20{''}$	&	$2.09$$\pm^{0.90}_{0.97}$\\ 
42  	&	ILTJ104430.59+585518.4	&	$10^{\mathrm{h}}44^{\mathrm{m}}30.59^{\mathrm{s}}$	&	$+58^{\circ}55{'}15.90{''}$	&	$1.94$$\pm^{0.41}_{0.36}$\\ 
43  	&	ILTJ104730.66+590427.5	&	$10^{\mathrm{h}}47^{\mathrm{m}}30.73^{\mathrm{s}}$	&	$+59^{\circ} 4{'}22.50{''}$	&	$1.76$$\pm^{0.69}_{0.68}$\\ 
44  	&	ILTJ104601.72+590917.3	&	$10^{\mathrm{h}}46^{\mathrm{m}}1.99^{\mathrm{s}}$	&	$+59^{\circ} 9{'}18.20{''}$	&	$1.88$$\pm^{0.29}_{0.28}$\\ 
45  	&	ILTJ104731.18+591134.4	&	$10^{\mathrm{h}}47^{\mathrm{m}}29.72^{\mathrm{s}}$	&	$+59^{\circ}11{'}32.50{''}$	&	$  -  $ \\ 
46  	&	ILTJ104601.56+585153.4	&	$10^{\mathrm{h}}46^{\mathrm{m}}1.26^{\mathrm{s}}$	&	$+58^{\circ}51{'}52.20{''}$	&	$2.27$$\pm^{0.92}_{1.36}$\\ 
47 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}46^{\mathrm{m}}21.39^{\mathrm{s}}$	&	$+58^{\circ}54{'}34.10{''}$	&	$  -  $ \\ 
48 $^{\dagger}$	&	 	&	$10^{\mathrm{h}}44^{\mathrm{m}}18.32^{\mathrm{s}}$	&	$+59^{\circ} 2{'}41.30{''}$	&	$  -  $ \\ 
49  	&	ILTJ104744.66+591413.6	&	$10^{\mathrm{h}}47^{\mathrm{m}}44.16^{\mathrm{s}}$	&	$+59^{\circ}14{'}11.90{''}$	&	$2.20$$\pm^{0.58}_{0.53}$\\ 
50  	&	ILTJ104444.87+591500.9	&	$10^{\mathrm{h}}44^{\mathrm{m}}44.53^{\mathrm{s}}$	&	$+59^{\circ}14{'}50.50{''}$	&	$  -  $ \\ 
51* 	&	ILTJ104354.98+590616.7	&	$10^{\mathrm{h}}43^{\mathrm{m}}55.28^{\mathrm{s}}$	&	$+59^{\circ} 6{'}16.00{''}$	&	$2.84$$\pm^{0.86}_{0.82}$\\ 
52  	&	ILTJ104539.62+584829.8	&	$10^{\mathrm{h}}45^{\mathrm{m}}39.90^{\mathrm{s}}$	&	$+58^{\circ}48{'}30.00{''}$	&	$3.70$$\pm^{1.45}_{1.45}$\\ 
53  	&	ILTJ104738.02+585634.2	&	$10^{\mathrm{h}}47^{\mathrm{m}}37.65^{\mathrm{s}}$	&	$+58^{\circ}56{'}32.20{''}$	&	$  -  $ \\ 
\hline 


==> table_flux.tex <==
ID	&	S$_{850} $	&	S$_{150 \rm{MHz}} $	&	S$_{324 \rm{MHz}} $	&	S$_{610 \rm{MHz}} $	&	S$_{1.4 \rm{GHz}} $	&	$\alpha_{150-324}$	&	$\alpha_{324-1400}$			\\  
		& 	(mJy)		&	($\mu$Jy)			&	($\mu$Jy)			&	($\mu$Jy)			&	($\mu$Jy)			&						&								\\  
\hline 
1  	&	11.91$\pm$ 1.23	&	$515.87\pm 21.88$	&	$269.05\pm 74.19$	&	$215.36\pm 16.93$	&	$80.64\pm 3.72$	&	$-0.81$	&	$-0.82$\\ 
2  	&	12.28$\pm$ 0.00	&	$569.90\pm 45.00$	&	$326.56\pm 69.59$	&	$230.62\pm 18.62$	&	$60.12\pm 6.04$	&	$-0.69$	&	$-1.16$\\ 
3* 	&	9.91$\pm$ 1.33	&	$437.02\pm 84.05$	&	$218.79\pm 69.63$	&	$243.83\pm 34.52$	&	$76.62\pm 6.97$	&	$-0.86$	&	$-0.72$\\ 
4  	&	8.92$\pm$ 1.62	&	$627.80\pm 26.03$	&	$654.40\pm 67.81$	&	$463.67\pm 12.53$	&	$232.95\pm 3.45$	&	$0.05$	&	$-0.71$\\ 
5  	&	8.66$\pm$ 1.43	&	$260.40\pm 33.58$	&	$185.44\pm 65.30$	&	$97.98\pm 16.65$	&	$46.60\pm 4.08$	&	$-0.42$	&	$-0.94$\\ 
6  	&	9.68$\pm$ 0.91	&	$155.09\pm 28.09$	&	$226.77\pm 63.90$	&	$66.25\pm 14.25$	&	$32.53\pm 4.82$	&	$0.47$	&	$-1.33$\\ 
7  	&	8.15$\pm$ 1.28	&	$427.66\pm 30.85$	&	$318.65\pm 81.14$	&	$217.56\pm 15.91$	&	$119.51\pm 3.12$	&	$-0.37$	&	$-0.67$\\ 
8 $^{\dagger}$	&	8.31$\pm$ 1.50	&	$53.22\pm 217.11$	&	$-73.58\pm 306.52$	&	$39.84\pm 37.60$	&	$-21.12\pm 65.69$	&	$  -  $	&	$  -  $\\ 
9* 	&	7.92$\pm$ 1.37	&	$352.32\pm 24.68$	&	$242.35\pm 45.25$	&	$110.80\pm 11.23$	&	$36.95\pm 3.90$	&	$-0.47$	&	$-1.29$\\ 
10  	&	7.91$\pm$ 1.36	&	$2757.32\pm 29.80$	&	$1591.78\pm 65.92$	&	$923.99\pm 10.53$	&	$265.02\pm 4.33$	&	$-0.68$	&	$-1.23$\\ 
11  	&	8.92$\pm$ 1.35	&	$2901.79\pm 33.26$	&	$1886.64\pm 66.49$	&	$965.98\pm 8.66$	&	$261.03\pm 6.77$	&	$-0.54$	&	$-1.35$\\ 
12  	&	7.45$\pm$ 1.32	&	$891.28\pm 35.67$	&	$597.49\pm 64.44$	&	$314.52\pm 14.95$	&	$131.48\pm 4.16$	&	$-0.50$	&	$-1.03$\\ 
13  	&	7.35$\pm$ 1.33	&	$677.98\pm 25.79$	&	$399.62\pm 75.91$	&	$218.91\pm 11.76$	&	$65.99\pm 4.84$	&	$-0.66$	&	$-1.23$\\ 
14  	&	7.87$\pm$ 0.86	&	$382.77\pm 22.14$	&	$211.55\pm 78.58$	&	$173.30\pm 15.20$	&	$34.05\pm 6.29$	&	$-0.74$	&	$-1.25$\\ 
15  	&	7.56$\pm$ 1.40	&	$195.09\pm 82.58$	&	$-142.94\pm 252.32$	&	$76.64\pm 64.94$	&	$202.57\pm 69.16$	&	$  -  $	&	$  -  $\\ 
16 $^{\dagger}$	&	6.81$\pm$ 1.44	&	$147.40\pm 187.52$	&	$-136.26\pm 286.97$	&	$39.09\pm 33.00$	&	$-115.27\pm 52.75$	&	$  -  $	&	$  -  $\\ 
17* 	&	6.77$\pm$ 1.37	&	$396.25\pm 18.82$	&	$230.10\pm 75.84$	&	$155.23\pm 13.57$	&	$39.92\pm 3.66$	&	$-0.68$	&	$-1.20$\\ 
18  	&	6.76$\pm$ 1.42	&	$786.16\pm 36.80$	&	$611.55\pm 80.54$	&	$413.93\pm 14.34$	&	$205.57\pm 4.10$	&	$-0.31$	&	$-0.74$\\ 
19  	&	6.72$\pm$ 1.30	&	$257.25\pm 21.91$	&	$304.00\pm 75.83$	&	$68.13\pm 10.48$	&	$31.74\pm 4.65$	&	$0.21$	&	$-1.54$\\ 
20  	&	7.45$\pm$ 1.14	&	$201.01\pm 117.18$	&	$63.77$	&	$67.83\pm 48.35$	&	$-243.98\pm 90.86$	&	$  -  $	&	$  -  $\\ 
21  	&	6.45$\pm$ 1.36	&	$246.71\pm 25.95$	&	$170.03\pm 75.18$	&	$129.69\pm 9.11$	&	$55.18\pm 3.85$	&	$-0.46$	&	$-0.77$\\ 
22* 	&	8.25$\pm$ 1.51	&	$599.27\pm 68.02$	&	$349.86\pm 88.50$	&	$187.96\pm 53.06$	&	$30.08\pm 8.89$	&	$-0.67$	&	$-1.68$\\ 
23  	&	8.15$\pm$ 2.06	&	$306.75\pm 21.86$	&	$302.24\pm 70.87$	&	$123.97\pm 11.61$	&	$36.63\pm 6.55$	&	$-0.02$	&	$-1.44$\\ 
24* 	&	6.47$\pm$ 1.19	&	$611.65\pm 412.64$	&	$46.51\pm 349.55$	&	$179.32\pm 186.81$	&	$286.13\pm 50.29$	&	$  -  $	&	$  -  $\\ 
25  	&	6.31$\pm$ 1.36	&	$514.89\pm 26.75$	&	$248.83\pm 67.93$	&	$191.35\pm 9.75$	&	$67.50\pm 3.82$	&	$-0.90$	&	$-0.89$\\ 
26* 	&	6.50$\pm$ 1.39	&	$316.26\pm 44.95$	&	$200.46\pm 74.80$	&	$148.73\pm 19.29$	&	$45.82\pm 3.71$	&	$-0.57$	&	$-1.01$\\ 
27*$^{\dagger}$	&	6.32$\pm$ 1.57	&	$331.03\pm 103.48$	&	$314.05\pm 261.99$	&	$31.25\pm 55.27$	&	$456.51\pm 75.47$	&	$  -  $	&	$  -  $\\ 
28  	&	6.17$\pm$ 1.27	&	$280.43\pm 29.52$	&	$134.93\pm 53.37$	&	$122.89\pm 12.37$	&	$47.90\pm 4.63$	&	$-0.91$	&	$-0.71$\\ 
29  	&	8.84$\pm$ 1.68	&	$417.91\pm 25.87$	&	$208.33\pm 55.58$	&	$196.16\pm 14.54$	&	$55.21\pm 6.88$	&	$-0.87$	&	$-0.91$\\ 
30 $^{\dagger}$	&	6.42$\pm$ 1.52	&	$503.76\pm 114.80$	&	$781.95\pm 283.17$	&	$153.31\pm 75.00$	&	$420.91\pm 93.98$	&	$  -  $	&	$  -  $\\ 
31  	&	6.69$\pm$ 1.53	&	$214.44\pm 18.08$	&	$203.56\pm 82.41$	&	$77.61\pm 16.35$	&	$25.53\pm 6.76$	&	$-0.06$	&	$-1.42$\\ 
32* 	&	5.52$\pm$ 1.21	&	$197.99\pm 37.48$	&	$186.59\pm 115.89$	&	$105.71\pm 69.49$	&	$32.39\pm 3.22$	&	$-0.07$	&	$-1.20$\\ 
33  	&	6.30$\pm$ 1.33	&	$320.15\pm 33.35$	&	$182.35\pm 47.71$	&	$111.52\pm 17.30$	&	$45.49\pm 6.72$	&	$-0.70$	&	$-0.95$\\ 
34* 	&	5.44$\pm$ 1.30	&	$224.34\pm 52.19$	&	$245.03\pm 77.06$	&	$56.77\pm 21.37$	&	$39.70\pm 5.24$	&	$0.11$	&	$-1.24$\\ 
35  	&	5.50$\pm$ 1.33	&	$603.71\pm 32.53$	&	$367.44\pm 71.91$	&	$283.81\pm 15.07$	&	$129.00\pm 3.86$	&	$-0.62$	&	$-0.72$\\ 
36  	&	5.42$\pm$ 1.18	&	$799.27\pm 254.92$	&	$164.88\pm 326.85$	&	$329.11\pm 256.36$	&	$368.81\pm 58.78$	&	$  -  $	&	$  -  $\\ 
37 $^{\dagger}$	&	4.86$\pm$ 1.29	&	$520.94\pm 83.10$	&	$-29.62\pm 313.97$	&	$136.86\pm 60.50$	&	$130.38\pm 48.72$	&	$  -  $	&	$  -  $\\ 
38  	&	6.37$\pm$ 1.38	&	$748.04\pm 128.77$	&	$232.76$	&	$45.05\pm 53.30$	&	$124.80\pm 119.67$	&	$  -  $	&	$  -  $\\ 
39  	&	4.98$\pm$ 1.33	&	$290.25\pm 33.77$	&	$315.02\pm 75.94$	&	$153.90\pm 8.45$	&	$53.63\pm 4.57$	&	$0.10$	&	$-1.21$\\ 
40 $^{\dagger}$	&	5.07$\pm$ 1.20	&	$67.59\pm 98.51$	&	$-341.11\pm 221.77$	&	$99.69\pm 42.18$	&	$20.18\pm 59.61$	&	$  -  $	&	$  -  $\\ 
41  	&	5.05$\pm$ 1.31	&	$1276.44\pm 27.34$	&	$786.63\pm 65.59$	&	$447.18\pm 12.20$	&	$189.72\pm 2.92$	&	$-0.60$	&	$-0.97$\\ 
42  	&	5.25$\pm$ 1.39	&	$475.66\pm 28.96$	&	$181.98\pm 63.07$	&	$192.92\pm 8.36$	&	$44.27\pm 4.53$	&	$-1.20$	&	$-0.97$\\ 
43  	&	5.02$\pm$ 1.28	&	$341.40\pm 26.43$	&	$331.18\pm 66.97$	&	$162.85\pm 11.18$	&	$65.27\pm 4.43$	&	$-0.04$	&	$-1.11$\\ 
44  	&	4.73$\pm$ 1.19	&	$464.62\pm 40.36$	&	$345.32\pm 85.46$	&	$193.13\pm 10.54$	&	$64.20\pm 3.66$	&	$-0.37$	&	$-1.15$\\ 
45  	&	5.31$\pm$ 1.43	&	$76.03\pm 239.46$	&	$-19.76\pm 232.55$	&	$164.37\pm 84.16$	&	$139.95\pm 95.10$	&	$  -  $	&	$  -  $\\ 
46  	&	4.53$\pm$ 1.14	&	$516.47\pm 25.07$	&	$297.33\pm 74.08$	&	$222.81\pm 9.71$	&	$116.54\pm 3.86$	&	$-0.69$	&	$-0.64$\\ 
47 $^{\dagger}$	&	4.66$\pm$ 1.15	&	$-106.75\pm 81.23$	&	$32.22\pm 250.29$	&	$-10.28\pm 49.18$	&	$93.86\pm 52.67$	&	$  -  $	&	$  -  $\\ 
48 $^{\dagger}$	&	5.00$\pm$ 1.51	&	$271.83\pm 80.87$	&	$-131.63$	&	$60.10\pm 51.23$	&	$-119.05\pm 67.70$	&	$  -  $	&	$  -  $\\ 
49  	&	5.89$\pm$ 1.28	&	$197.55\pm 24.97$	&	$150.22\pm 68.25$	&	$104.23\pm 16.23$	&	$40.82\pm 7.98$	&	$-0.34$	&	$-0.89$\\ 
50  	&	6.40$\pm$ 1.59	&	$452.53\pm 200.45$	&	$174.61\pm 244.19$	&	$173.99\pm 69.35$	&	$49.36\pm 105.88$	&	$  -  $	&	$  -  $\\ 
51* 	&	6.04$\pm$ 1.76	&	$332.04\pm 66.28$	&	$231.01\pm 91.76$	&	$145.52\pm 40.04$	&	$51.86\pm 8.26$	&	$-0.45$	&	$-1.02$\\ 
52  	&	4.60$\pm$ 1.30	&	$323.68\pm 27.13$	&	$252.34\pm 69.15$	&	$187.14\pm 11.54$	&	$67.46\pm 4.56$	&	$-0.31$	&	$-0.90$\\ 
53  	&	4.59$\pm$ 1.19	&	$402.38\pm 97.36$	&	$43.27\pm 273.87$	&	$61.92\pm 42.72$	&	$-30.77\pm 74.99$	&	$  -  $	&	$  -  $\\ 
\hline 

